A Novel Membership Inference Attack against Dynamic Neural Networks by Utilizing Policy Networks Information

Unlike traditional static deep neural networks (DNNs), dynamic neural networks (NNs) adjust their structures or parameters to different inputs to guarantee accuracy and computational efficiency. Meanwhile, it has been an emerging research area in deep learning recently. Although traditional static DNNs are vulnerable to the membership inference attack (MIA) , which aims to infer whether a particular point was used to train the model, little is known about how such an attack performs on the dynamic NNs. In this paper, we propose a novel MI attack against dynamic NNs, leveraging the unique policy networks mechanism of dynamic NNs to increase the effectiveness of membership inference. We conducted extensive experiments using two dynamic NNs, i.e., GaterNet, BlockDrop, on four mainstream image classification tasks, i.e., CIFAR-10, CIFAR-100, STL-10, and GTSRB. The evaluation results demonstrate that the control-flow information can significantly promote the MIA. Based on backbone-finetuning and information-fusion, our method achieves better results than baseline attack and traditional attack using intermediate information.

==> sections/Defense.tex <==
% \section{Defense by Filterring}



==> sections/Relatedwork.tex <==
\section{Related Work}


\subsection{Backdoor Attack and Defense} 
\label{subsec:backdoor attack and defense}
BadNets~\cite{gu2017badnets} first introduce a backdoor attack into DNNs, which pollutes the training dataset with some poisoned data stamped with triggers (e.g., $3 \times 3$ white square in the lower right corner of the image) and mislabels them as the target label. Then, the polluted dataset is fed into DNNs to train the victim model, which finally will misclassify the instances stamped with the trigger as the target label. However, BadNets needs to access the original dataset to poison and control the training of models, which is not always possible. In contrast, Trojaning Attack~\cite{liu2017trojaning} proposes to generate a general trigger by reversing the victim DNN and retraining the DNN with the generated dataset containing poisoned instances stamped with the reversed trigger to inject backdoors. However, Trojaning attack needs to reverse one image for each label to generate the dataset and fine-tune all parameters, which is too costly on large models with many parameters and labels, such as ViT-G/14~\cite{Zhai2021ScalingVT} (two billion parameters) trained on JFT-3B dataset (30k labels). Our backdoor attack consumes much fewer resources and can embed backdoors in a data-free manner. 
Moreover, there are several backdoor attacks in the NLP tasks. Kurita et al.~\cite{kurita2020weight} propose to construct ``weight poisoning'' attack to inject a backdoor into pre-trained NLP models. BadNL~\cite{chen2021badnl}  performs a systematic investigation of backdoor attack on
NLP models and proposes
three methods to construct triggers, namely BadChar, BadWord,
and BadSentence. Moreover, Yang et al.~\cite{yang2021rethinking} propose a stealthy backdoor attack based on negative data augmentation and modifying word embeddings. However, the work mentioned above requires access to the training dataset and does not apply to data-free scenarios.

% there are also some work related to the NLP task~\cite{fan2021text,chen2021badnl,yang2021rethinking}.

Neural Cleanse~\cite{wang2019neural} determines whether a DNN model is infected by reversing the potential trigger patterns towards each class and identifying the real trigger and its label based on outlier detection. Unfortunately, Neural Cleanse may consume too much resource for the models with numerous parameters and labels. 
TABOR~\cite{Guo2019TABORAH} further improves the performance of reversing triggers via various regularizations during optimizations, leading to more computation resource consumption than Neural Cleanse. Furthermore, Chen et al. propose DeepInspect~\cite{chen2019deepinspect} to detect the backdoor attack. It first generated training data by reverse engineering and then used a conditional generative model to learn the probabilistic distribution of potential triggers to generate triggers.
ABS~\cite{Liu2019ABSSN} proposes to find the neurons contributing to the backdoors based on the assumption that the neurons that substantially elevate the activation of a particular output label regardless of the provided inputs are considered potentially compromised. However, it may not be suitable for large models with numerous neurons due to the training cost.
Moreover, both SentiNet~\cite{chou2018sentinet} and Februus~\cite{doan2020februus} utilize Grad-GAM~\cite{selvaraju2017grad} to discover the contiguous regions of an input image that contribute significantly to the classification result and conclude that such regions are highly likely to contain a trigger. Generally, we can improve our attack's resistance against various defense approaches by adding the adaptive loss during the backdoor injection, as discussed in Section~\ref{sec:discussion}.

\subsection{Adversarial Attack against Transformers}
The adversarial attack represents the attack technique that exploits available model information and uses it to create adversarial examples to make the model misclassify. Aldahdooh et. al. ~\cite{Aldahdooh2021RoV} study the robustness of vision transformers and their variants and compare them with CNNs and find that either vanilla ViTs or hybrid-ViTs are more robust than CNNs against $L_{p}$-based adversarial attacks and color channel perturbations (CCP) attacks. Mahmood et. al.~\cite{Mahmood2021OnTR} study the robustness of Vision Transformers against adversarial attacks and show that adversarial examples do not transfer well between CNNs and transformers. Naseer et. al. investigate the weak transferability of adversarial patterns on ViT models and propose transferable attacks based on multiple discriminative pathways, and token refinement \cite{Naseer2021OnIA}. And Wei et. al.~\cite{Wei2021ToTr} posit that adversarial attacks on transformers should be specially tailored for their architecture and introduce a dual attack framework, which contains a Pay No Attention (PNA) attack and a PatchOut attack, to improve the transferability of adversarial samples across different ViTs. Moreover, Joshi et. al.~\cite{Joshi2021AdversarialTA} design an adversarial token attack and find that transformer model are more sensitive to token attacks than classic convolutional models. Mao et. al.~\cite{Mao2021TowardsRV} propose Robust Vision Transformer (RVT) by evaluating robust components of ViT to adversarial examples and combining them as building blocks of RVT. 
And Sahu et. al.~\cite{Sahu2021EnTr} introduced Gated Adversarial Transformer (GAT) to enhance the applicability of attention-based models in the videos area and also proposed a temporal attention regularization scheme to improve the robustness of attention modules to adversarial examples.

\iffalse
For each transformer block, we can get a Raw Attention Matrix $A_{ij}$ that defines how much attention is going to flow from token $j$ in the previous layer to token $i$ in the next layer. Particularly, the Raw Attention is calculated as below:

\begin{equation}
A = softmax(qk^{T}/\sqrt{D_{h}})
\end{equation}
where $q$ and $k$ represents query and key respectively, $D_{h}$ represents the dimension of query and key.  

\noindent\textbf{Attention Rollout}
Unlike Raw Attention, Attention Rollout aims to get the attention flowing from the images to the target layer. Owning to residual connections, we need to add the identity matrix $I$ to the layer Attention matrices: $A_{ij}+I$.
We can multiply the matrices between every two layers to get the total attention flow between them, so we get a way to compute the Attention Rollout matrix at layer $L$ recursively:

\begin{equation}
\tilde{A}_{L} = \begin{cases}
(A_{L}+I)\tilde{A}_{L-1}, & L>0 \\
A_{L}+I,& L=0 \\
\end{cases}
\end{equation}
where $\tilde{A}_{L}$ is the Attention Rollout, $A$ represents the Raw Attention.
\fi

